D2.1 Models for energy consumption of data structures and algorithms

This deliverable reports our early energy models for data structures and algorithms based on both micro-benchmarks and concurrent algorithms. It reports the early results of Task 2.1 on investigating and modeling the trade-off between energy and performance in concurrent data structures and algorithms, which forms the basis for the whole work package 2 (WP2). The work has been conducted on the two main EXCESS platforms: (1) Intel platform with recent Intel multi-core CPUs and (2) Movidius embedded platform.

==> D2.1-microbench.tex <==
\newcommand{\pcaA}{\ema{A}}       %power constant
\newcommand{\pcbA}{\ema{B}}       %power constant
\newcommand{\pceA}{\ema{\alpha}}  %power exponent
\newcommand{\pceoA}{\ema{\alpha_0}}  %power exponent

\newcommand{\freqA}{\ema{freq}}
\newcommand{\freqB}{\ema{\mathit{freq}}}

\subsubsection{Microbenchmark for CPU}

\paragraph{Power Model}

The power model, that is presented in the D1.1, decomposes the total power into static, socket activation and dynamic
power. For modeling power consumption of data-structures, we need to estimate the dynamic component which depends
on the frequency, number of active cores, locality and amount of memory requests together with the instruction type
as also mentioned in the D1.1. 
To improve the our previous power model given in equation~\ref{eq.power-model-micro}, we applied an orthogonal
power decomposition including cpu, uncore and memory components, that are provided by RAPL energy counters, to
each component as illustrated in the figure~\ref{fig.pow-dec-micro}. This additional orthogonal dimension will
provide a better perspective to model power consumption of data-structures, especially for the dynamic component.

\begin{equation}
P(\freq,\prog,\pin,\mathit{threads}) = \pstat{}  + \#\{\mathrm{active~sockets}\} \times \pact{} (f)
             + \pdyn{} (f,\prog,\pin,\mathit{threads}).
\label{eq.power-model-micro}
\end{equation}

\begin{figure} [h!]
\begin{center}
\begin{tabular}{|c|c|c|c|}
%\hline
\cline{2-4}
\multicolumn{1}{c|}{}&        Static & Active & Dynamic\\\hline
CPU    & \pstat{C} & \pact{C} & \pdyn{C} \\\hline
Memory & \pstat{M} & \pact{M} & \pdyn{M} \\\hline
Uncore & \pstat{U} & \pact{U} & \pdyn{U} \\\hline
\end{tabular}
\end{center}
\caption{Power views\label{fig.pow-dec-micro}}
\end{figure}

Thus, we define the total power by using 2 orthogonal decomposition:

\[ P(\freq,\prog,\pin,\mathit{threads}) = \sum_{X \in \{C,M,U\}} \left( \pstat{X} +
\#\{\mathrm{active~sockets}\} \times \pact{X} + \pdyn{X}  \right). \]


\paragraph{Power Components Derivation}

By definition, only the dynamic component of power is dependent to type of instruction or equally the executing 
program. In order to obtain dynamic component, we first have to determine static and socket activation costs.
This was done in D1.1 but the derivation process was not described in detail. Therefore, we will explain it
briefly in this subsection. 

In the D1.1, a large variety of instructions were examined with respect to their power and energy consumption.
We observed a linear relation between the number of threads and power for instructions when operands of 
instructions are independent for each thread. Briefly, we make use of this fact to obtain static and socket
activation costs for each component (cpu, memory, uncore) of orthogonal decomposition. Bunch of instructions belonging
to this class is executed repeatedly for some time interval with
varying number of threads for each frequency. Pinning does not have an impact on the dynamic component of power
for such instructions since there is no resource sharing between threads. We formulated the derivation process as:

\begin{multline*}
 \pdyn{X\in \{C,M,U\}}(\freq,\prog,\pin,\mathit{threads}) = \\
\frac{\mathit{threads}\times(P^{(X\in \{C,M,U\})})(\freq,\prog,\mathit{dense},16) - P^{(X\in \{C,M,U\})}(\freq,\prog,\mathit{dense},14))}{2}
\end{multline*}

\begin{multline*}
 \pact{X\in \{C,M,U\}}(\freq,\prog,\pin,\mathit{threads}) = \\
P^{(X\in \{C,M,U\})}(\freq,\prog,\mathit{dense},10) -
P^{(X\in \{C,M,U\})}(\freq,\prog,\mathit{dense},8) - \pdyn{X\in \{C,M,U\}}(\freq,\prog,\pin,2)
\end{multline*}


\begin{multline*}
 \pstat{X\in \{C,M,U\}}(\freq,\prog,\pin,\mathit{threads}) = \\
P^{(X\in \{C,M,U\})})(\freq,\prog,\pin,\mathit{threads}) - \\ 
\pact{X\in \{C,M,U\}}(\freq,\prog,\pin,\mathit{threads}) - \\
\pdyn{X\in \{C,M,U\}}(\freq,\prog,\pin,\mathit{threads})
\end{multline*}


Using above equations, we verified that
$\pstat{X\in \{C,M,U\}})$ does not depend on
instruction type, pinning, number of threads and frequency. The values for each combination is very close so
we take the mean to find the \pstat{} in terms of orthogonal components \pact{X\in \{C,M,U\}}. We applied the same
approach to find the $\pact{X\in \{C,M,U\}}$ which only depends on frequency. 
We provide a socket value for each frequency again by taking mean on other dimensions.
Having obtained \pstat{} and \pact{}, we extracted the \pdyn{X\in \{C,M,U\}}
for ``all`` types of instructions, thread, pinning and frequency setting. 

\paragraph{Dynamic Cpu Power}

\newcommand{\alf}{\ema{\alpha}}  %power exponent
\newcommand{\A}{\ema{A}}       %power constant
\newcommand{\B}{\ema{B}}       %power constant

Having determined and excluded static and socket components, we obtained the dynamic power component for each
instruction, thread count, pinning and frequency setting. In the microbenchmarks for D1.1, a large variety of
instructions are surveyed. Among them, we picked a small set of instructions that can be representative for
data-structure implementations, namely \cas, pause, floating point division, addition together with vector addition.
\cas can be representative for the retry loops and division/additions can be used to represent the parallel work which
determines the contention on the data-structures. The decomposition of dynamic power in terms of cpu,
memory and uncore components for these instructions are illustrated in the
figures~\ref{fig.cpu_dyn_micro},~\ref{fig.mem_dyn_micro} and~\ref{fig.uncore_dyn_micro}.

\begin{figure} [h!]
\includegraphics[width=\textwidth]{cpu_dyn_microbench}
\caption{Cpu dynamic power for microbenchmarks\label{fig.cpu_dyn_micro}}
\end{figure}

Based on the observation that \pdyn{C} shows almost linear behavior with respect to number of threads, we modeled
the convex \pdyn{C} as:  

\[ \mathit{threads} \times \left( \A \times \freq^{\alf} + \B \right) \]

Each instruction might provide different power behavior as illustrated in the figure~\ref{fig.cpu_dyn_micro},
therefore we find \A, \B, \alf for each instruction separately. \B could be different for each instruction because
of the activation of different functional units, this is also why we included this constant in the \pdyn{C}. 

To obtain \A, \B and \alf, we solved the minimization problem: (with the help of Matlab ``fminsearch'' function)

\[ \forall \freq \in \{1.2, .., 3.4\} MIN(\pdyn{C} (\freq,\prog_0,\pin,\mathit{threads})
-  \mathit{threads} \times \left( \A \times \freq^{\alf} + \B \right))\]

Figure~\ref{fig.pow-coeff-micro} provides the values for power constants and exponent for selected instructions.

\begin{figure} [h!]
\begin{center}
\begin{tabular}{|c|c|c|c|}
%\hline
\cline{2-4}
\multicolumn{1}{c|}{}&        \A & \alf & \B \\\hline
cas   & 0.0014 & 1.6415 & 0.0510 \\\hline
fpdiv & 0.0010 & 1.7226 & 0.0585 \\\hline
add & 0.0010 & 1.8148 & 0.0912 \\\hline
avx-add & 0.0011 & 1.7828 & 0.0894 \\\hline
pause & 0.0009 & 1.7920 & 0.0736 \\\hline
\end{tabular}
\end{center}
\caption{Instruction power coefficients\label{fig.pow-coeff-micro}}
\end{figure}



\paragraph{Dynamic Memory and Uncore Power}

In the microbenchmarks, we observed that many instruction does not lead to an increase in dynamic memory
and uncore power. This is expected because operands of the instructions, except \cas, presumably resides in 
the L1 cache. On the other hand, \cas lead to an increase in memory and uncore power when the threads are pinned
to different sockets. The ping-pong of cache line between sockets is responsible from this effect.   
As mentioned in D1.1, \cas microbenchmarks are prone to unfairness among threads. When \cas is executed repeatedly
by all threads on the same cache line without any work in between \cas attempts, the thread which gets the ownership
of cache line succeeds repeatedly while others starve. This fact decreases the transfer rate of cache line between 
local caches. Due to this, we introduced 3 different \cas microbenchmarks each looping on 1,3 and 50 shared variables
that are aligned to different cache lines. By doing so, we aimed to increase the traffic between cores and sockets
together with amount of memory accesses. The figures~\ref{fig.mem_dyn_micro} and~\ref{fig.uncore_dyn_micro} provide
\pdyn{U} and \pdyn{M} values. It can be observed that all parameters including number of threads, frequency, pinning
play a role for \cas. As a remark for the provided figures, threads are pinned using a dense mapping strategy that
leads to intersocket communication only after 8 threads.

\begin{figure}[h!]
\includegraphics[width=\textwidth]{mem_dyn_microbench}
\caption{Memory dynamic power for microbenchmarks\label{fig.mem_dyn_micro}}
\end{figure}

\begin{figure}[h!]
\includegraphics[width=\textwidth]{uncore_dyn_microbench}
\caption{Uncore dynamic power for microbenchmarks\label{fig.uncore_dyn_micro}}
\end{figure}

\pdyn{U} and \pdyn{M} does not increase when threads are pinned to same socket. In this case, the intrasocket 
communication between threads takes place via the ring interconnect without introducing a memory access. Thus, absence
of increase in memory power is reasonable. However, one might expect an increase in uncore power for these cases
because RAPL uncore power presumably includes LLC and ring interconnect power. However, we do not observe this.
The increase of uncore and memory power can be observed when threads are pinned to different sockets, due to remote
memory accesses. An interesting observation regarding memory power is that it shows a step function behavior.  
We think that this is because of the RAPL power capping algorithm which determines a power budget based on
memory bandwidth, as presented in the work of David .et al~\ref{}. RAPL algorithm specifies a power cap for
a time window depending on the memory bandwidth requirements of previous time intervals and puts the memory in a power
state that is expected to maximize energy efficiency. Based on the amount memory accesses, it jumps between states
each providing a trade-off between bandwidth and power. Finite number of states leads to this step like power
curves~\ref{fig.mem_dyn_micro}. Thus, the memory power is determined by the amount of memory access per time
interval which is dependent to frequency, number of threads and the amount of shared variables for our \cas experiments.

All these observations regarding memory and uncore power will shed light to the analysis/modeling of data-structures
in the following sections. One major source of power consumption difference between different implementations is the
memory consumption which is related to locality and bandwidth requirements of implementations.




==> energy-analysis-models.tex <==
\remind{Chalmers: please fill this section}

==> energy-analysis-myriad1.tex <==
\subsection{Sanity Check of Movidius Power Model} 
The experiments are conducted for benchmarks with single unit and multiple units. Each benchmark is tested by running Myriad1 with  1, 2, 4, 6 and 8 SHAVE cores.

From the experiment results, we observe that the power consumption of Movidius Myriad1 platform is ruled by the following model:
\begin{equation} \label{eq:Pfirst}
	P=P^{stat}+\#\{\text{active shave}\} \times (P^{act}+P^{dyn}_{shave})
\end{equation}
The operands in the formula are explained as below.
The static power $p^{stat}$ is the needed power when the Myriad1 processor is on. The $p^{act}$ is the power consumed when a SHAVE core is on. Therefore, this active power is multiplied with number of used SHAVE core when the benchmark is run with several cores. 

The dynamic power $P^{dyn}_{shave}$ of each SHAVE is the power consumed by all working operation units working on SHAVE. As described in the previous section, each SHAVE core has several components, including LSU, PEU, BRU, IAU, SAU, VAU, CMU, etc. Different arithmetic operation units have different $p^{dyn}$ values. In this power model, we focus on the experiments with the benchmarks performing different arithmetic operations such as IAU, VAU, SAU and CMU.  

The dynamic power $p^{dyn}$ of each SHAVE is the power consumed by all working operation units. As described in the previous section, each SHAVE core has several components, including LSU, PEU, BRU, IAU, SAU, VAU, CMU, etc. Different arithmetic operation units have different $p^{dyn}$ values. In this power model, we focus on the experiments with the benchmarks performing different arithmetic operations such as IAU, VAU, SAU and CMU.  

%If the benchmark requires more than two units running on the same SHAVE core, this combined $p^{dyn}$ is computed by the sum of the $p^{dyn}$  of every unit in the combination. E.g. $p^{dyn}$ of SauXorVauMul = $p^{dyn}$ of SauXor + $p^{dyn}$ of VauMul.


When  adding one more shave, we can identify the sum of SHAVE $p^{act}$ and $p^{dyn}$ which is the power level difference of the two runs (with one shave core and with two shave core).  Given the sum of $p^{act}$ and $p^{dyn}$, $p^{stat}$ is derived from the formula. The experiment results show the average value of $p^{stat}$ from all experiment results:
\begin{equation} \label{eq:Pstat}
	P^{stat}=62.63 \text{ mW}
\end{equation}
Then for each operation unit, we obtain the two parameters $P^{dyn}_{op}$ and $p^{act}$ by using the actual power consumption of the benchmark for individual units and multiple units. 
\begin{equation} \label{eq:Pcomb}
	\begin{cases}
		P^{dyn}_{(IauXor)} =P^{stat} + \#\{\text{active shave}\} \times (P^{act}+P^{dyn}_{(IauXor)}) \\
		P^{dyn}_{(SauXorIauXor)}= P^{stat} + \#\{\text{active shave}\} \times (P^{act}+P^{dyn}_{(SauXorIauXor)})\\
		P^{dyn}_{(SauXor)}= P^{stat} + \#\{\text{active shave}\} \times (P^{act}+P^{dyn}_{(SauXor)})
	\end{cases}
\end{equation}

Then, the average value of  $p^{act}$ among all operation units is calculated.
\begin{equation} \label{eq:Pact}
	P^{act}=51.4 \text{ mW}
\end{equation}

At this point, we also have the $P^{dyn}_{op}$ of every arithmetic units. Applying the model to calculate the consumed energy, the results after plotting show the deviation from the measured data, especially the benchmarks running a single arithmetic unit. We attribute this difference to the inter-operation cost when more than one unit of SHAVE core work in a combination. This inter-operation cost is also mentioned in the model suggested by Movidius in EXCESS release D4.1 document. The $p^{dyn}$ of SHAVE running multiple units is then computed by the formula below:
\begin{equation} \label{eq:Pdynshave}
	P^{dyn}_{shave}=\sum_i{P^{dyn}_i(op)} + \max_i\{O_i(op)\}
\end{equation}

The combined $p^{dyn}$ is the sum of $p^{dyn}$ of each unit, plus the highest inter-operational cost $O_i$ among the unit in the combination. E.g. 
$P^{dyn}_{(SauXorIauXor)}) = P^{dyn}_{(SauXor)} + P^{dyn}_{(IauXor)} + \max(O_{SauXor}, O_{IauXor})$.

Given the $p^{stat}$ and $p^{act}$, the $P^{dyn}_{op}$ of an operation unit is computed based on the actual power consumption of the benchmark using a single unit(e.g. SauXor, IauXor, etc.). Then, its inter-operational cost is computed based on the actual power consumption when this unit works in a combination with other units.

The table~\ref{table:InteroperationalCost} lists the inter-operational cost of each unit when it works in a combination with other units.

\begin{table}[h]
\begin{center}
\begin{tabular}{|l|l|l|}
\hline
\textbf{Operation Unit} & \textbf{$P^{dyn}_{op}$} & \textbf{$O_{op}$} \\ \hline
SauXor                  & 3.05          & 1.15       \\ \hline
SauMul                  & 6.97          & 1.83       \\ \hline
VauXor                  & 17.57         & 13.12      \\ \hline
VaulMul                 & 32.78         & 11.62      \\ \hline
IauXor                  & 4.53          & 1.07       \\ \hline
IauMul                  & 3.98          & 4.42       \\ \hline
CmuCpss                 & 1.00          & 4.60       \\ \hline
CmuCpivr                & 6.41          & 5.69       \\ \hline
\end{tabular}
\caption{Inter-operational Cost of SHAVE Operation Units}
\label{table:InteroperationalCost}
\end{center}
\end{table}

From equations~\ref{eq:Pstat},~\ref{eq:Pact} and~\ref{eq:Pdynshave}, the complete model for Movidius Myriad1 is derived as follows:
\begin{equation} \label{eq:Psecond}
	P=P^{stat}+ \#\{\text{active shave}\} \times (P^{act}) + \#\{\text{active shave}\} \times \left( \sum_i{P^{dyn}_i(op)} + \max_i\{O_i(op)\} \right)
\end{equation}

Applying this formula to different combinations of operation units in SHAVE core, we plot the relative error of this model in the figure~\ref{fig:ErrorRelative}. The relative error is the difference between the actual power consumption measure by device and the predicted power consumption computed through Equation with parameter values from equation 1,2 and table 3, then divided by the actual power consumption. 
Under this model, the relative error varies from  -4\%-3\% which is 7\% margin. This model is not only applicable for a single unit but also the combination of two or three units.

\begin{figure}
\begin{center}
\includegraphics[width=0.9\textwidth]{Pics/PowerMeasurement/ErrorRelative.png}
\end{center}
%\vspace{-40pt}
\caption{Relative Error of Myriad1 Power Prediction}
\label{fig:ErrorRelative}
\end{figure}


==> energy-analysis-trees.tex <==
Energy consumption for each trees are calculated using the Excess cluster located in HLRS,
University of Stuttgart. The compute node of the cluster is equipped with
2x Intel Xeon E5-2690 v2 with 20 cores total. The available memory is 32GB 
(8 x 4GB) DDR3. This server is equipped with 4 x A/D converter that can measures 
the energy for each CPU+DRAM, PCIe, GPU, and PSU in real-time. Energy data were derived from the raw energy information coupled with specific time markers  in microsecond precision before the start of each threaded benchmarks. The calculated energy is the energy that was recorded after this specific marker timestamp. We did this to made sure that initialization activities will 
not add to the resulting energy calculation.

These benchmarks was done using similar setup of the performance benchmark 
with the exception that we tested only the extreme cases which are the combination of
0 and 20 threads and 0\% and 50\% updates (cf. Figure \ref{fig:energy-4m}).

\begin{figure}[!t] \centering
%\resizebox{\textwidth}{!}{
%	\includegraphics{figures/init4m}
%	\includegraphics{figures/init4m2}
%	}
%
%\resizebox{\textwidth}{!}{
%	\includegraphics{figures/init4m3}
%	\includegraphics{figures/init4m4}
%	}

%\includegraphics{figures/x86-power.eps}
\includegraphics{figures/x86-power-eps-converted-to.pdf}
\caption{Energy consumption of the tested trees with 4,194,303 initial members.}
\label{fig:energy-4m}
\vspace{-6pt}
\end{figure}



==> energy-modeling-queues-2.tex <==
\subsubsection{Benchmarks}

The benchmark is pictured in Algorithm~\ref{algo.queue-bench}.


\begin{figure}
\begin{algorithmic}[1]
%\SetAlgoLined

\State Initialization()\;
\While{execution time $<$ t}

	\State Parallel\_Work()\;

	\State Enqueue()\;

	\State Parallel\_Work()\;

	\State Dequeue()\;
\EndWhile

\end{algorithmic}
\caption{Queue benchmark}\label{algo.queue-bench}
%\label{fig.queue-bench}
%\caption{Queue benchmark}
\end{figure}

\paragraph{Throughput model}


The idea is to decompose the set of executions into two different
behaviors: congested and non-congested. Within the non-congested
behavior, the throughput can be computed as:
\[ \thr = \frac{\nth}{\beta \times (\cw + \pw)}, \]
where \thr is the throughput (\ie the number of successful enqueue or
dequeue per second), \nth is the number of threads that are working on
the queue, \cw (for critical work) is the work needed to either
enqueue or dequeue an element (we assume that those two amounts of
work are similar), \pw (for parallel work) is the amount of work
inside the \ema{\mathit{Parallel\_Work}} function, and $\beta$, which
depends on the frequency of the core, pictures the scalability of
those critical and parallel section with the frequency.

Within the congested state, the throughput is given by:
\[ \thr = a + \pw \times b. \]

For a given number of threads and a given implementation, we take
three points to estimate the parameters in the throughput model of the
congested state (small parallel work).

For a given implementation, we take two points to instantiate the
throughput model of the non-congested state (big parallel work).

For a given implementation and a given number of threads, when
plotting those two functions according to the size of the parallel
work, the final throughput estimate is taken as the throughput of
congested state for small parallel work sizes and of non-congested
state for big parallel work sizes; when the two curves intersect, we
go from a state to another. The result is depicted in
Figure~\ref{fig.est-through}.

One graph corresponds to a given number of threads (top number), and a
given frequency (right number). Each color is associated with an
implementation. The points are the measured throughputs, while the
lines are the throughput estimates.

\begin{figure}
\includegraphics[width=\textwidth]{queues/first_est_through}
\label{fig.est-through}
\caption{Throughput estimate}
\end{figure}


\paragraph{Power Model}

Same model as in D1.1.



The power consumption of the CPUs, when they execute a program \prog
in steady-state on a socket that runs at frequency $f$, is ruled by
the following model:
\begin{equation}
P(f,\prog,\pin) = \pstat + \#\{\mathrm{active~sockets}\} \times \pact(f)
             + \#\{\mathrm{active~cores}\} \times \pdyn(f,\prog).
\label{eq.power-model}
\end{equation}


\paragraph{Other implied metrics}

Now the top numbers are the sizes of the parallel work, and the right
numbers are still the frequency. See Figure~\ref{fig.est_energy_pop}.

\begin{figure}
\includegraphics[width=\textwidth]{queues/first_est_energy_pop}
\label{fig.est_energy_pop}
\caption{Energy per operation estimate}
\end{figure}



==> figures/perf-2097151.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,4320.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(976,2672){\makebox(0,0)[r]{\strut{}$0.0*10^{0}$}}%
      \put(976,2854){\makebox(0,0)[r]{\strut{}$5.0*10^{5}$}}%
      \put(976,3036){\makebox(0,0)[r]{\strut{}$1.0*10^{6}$}}%
      \put(976,3218){\makebox(0,0)[r]{\strut{}$1.5*10^{6}$}}%
      \put(976,3400){\makebox(0,0)[r]{\strut{}$2.0*10^{6}$}}%
      \put(976,3581){\makebox(0,0)[r]{\strut{}$2.5*10^{6}$}}%
      \put(976,3763){\makebox(0,0)[r]{\strut{}$3.0*10^{6}$}}%
      \put(976,3945){\makebox(0,0)[r]{\strut{}$3.5*10^{6}$}}%
      \put(976,4127){\makebox(0,0)[r]{\strut{}$4.0*10^{6}$}}%
      \put(1072,2512){\makebox(0,0){\strut{} 1}}%
      \put(1818,2512){\makebox(0,0){\strut{} 2}}%
      \put(2565,2512){\makebox(0,0){\strut{} 3}}%
      \put(3311,2512){\makebox(0,0){\strut{} 4}}%
      \put(128,3399){\rotatebox{-270}{\makebox(0,0){\strut{}operations/second}}}%
      \put(2191,2272){\makebox(0,0){\strut{}nr. of threads}}%
      \put(1184,3909){\makebox(0,0)[l]{\strut{}100\% Search}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(4576,2672){\makebox(0,0)[r]{\strut{}$0.0*10^{0}$}}%
      \put(4576,2880){\makebox(0,0)[r]{\strut{}$5.0*10^{5}$}}%
      \put(4576,3088){\makebox(0,0)[r]{\strut{}$1.0*10^{6}$}}%
      \put(4576,3296){\makebox(0,0)[r]{\strut{}$1.5*10^{6}$}}%
      \put(4576,3503){\makebox(0,0)[r]{\strut{}$2.0*10^{6}$}}%
      \put(4576,3711){\makebox(0,0)[r]{\strut{}$2.5*10^{6}$}}%
      \put(4576,3919){\makebox(0,0)[r]{\strut{}$3.0*10^{6}$}}%
      \put(4576,4127){\makebox(0,0)[r]{\strut{}$3.5*10^{6}$}}%
      \put(4672,2512){\makebox(0,0){\strut{} 1}}%
      \put(5418,2512){\makebox(0,0){\strut{} 2}}%
      \put(6165,2512){\makebox(0,0){\strut{} 3}}%
      \put(6911,2512){\makebox(0,0){\strut{} 4}}%
      \put(3728,3399){\rotatebox{-270}{\makebox(0,0){\strut{}operations/second}}}%
      \put(5791,2272){\makebox(0,0){\strut{}nr. of threads}}%
      \put(4784,3909){\makebox(0,0)[l]{\strut{}20\% Update}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(976,512){\makebox(0,0)[r]{\strut{}$0.0*10^{0}$}}%
      \put(976,803){\makebox(0,0)[r]{\strut{}$5.0*10^{5}$}}%
      \put(976,1094){\makebox(0,0)[r]{\strut{}$1.0*10^{6}$}}%
      \put(976,1386){\makebox(0,0)[r]{\strut{}$1.5*10^{6}$}}%
      \put(976,1677){\makebox(0,0)[r]{\strut{}$2.0*10^{6}$}}%
      \put(976,1968){\makebox(0,0)[r]{\strut{}$2.5*10^{6}$}}%
      \put(1072,352){\makebox(0,0){\strut{} 1}}%
      \put(1818,352){\makebox(0,0){\strut{} 2}}%
      \put(2565,352){\makebox(0,0){\strut{} 3}}%
      \put(3311,352){\makebox(0,0){\strut{} 4}}%
      \put(128,1240){\rotatebox{-270}{\makebox(0,0){\strut{}operations/second}}}%
      \put(2191,112){\makebox(0,0){\strut{}nr. of threads}}%
      \put(1184,1750){\makebox(0,0)[l]{\strut{}50\% Update}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(6195,1745){\makebox(0,0)[r]{\strut{}$\Delta$Tree}}%
      \csname LTb\endcsname%
      \put(6195,1585){\makebox(0,0)[r]{\strut{}CBtree}}%
      \csname LTb\endcsname%
      \put(6195,1425){\makebox(0,0)[r]{\strut{}b$\Delta$Tree}}%
      \csname LTb\endcsname%
      \put(6195,1265){\makebox(0,0)[r]{\strut{}h$\Delta$Tree}}%
      \csname LTb\endcsname%
      \put(6195,1105){\makebox(0,0)[r]{\strut{}rbtree}}%
      \csname LTb\endcsname%
      \put(6195,945){\makebox(0,0)[r]{\strut{}avltree}}%
      \csname LTb\endcsname%
      \put(6195,785){\makebox(0,0)[r]{\strut{}sftree}}%
      \csname LTb\endcsname%
      \put(6195,625){\makebox(0,0)[r]{\strut{}NBBST}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./perf-2097151-convert}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/perf-4194303.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,4320.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(976,2672){\makebox(0,0)[r]{\strut{}$0.0*10^{0}$}}%
      \put(976,2854){\makebox(0,0)[r]{\strut{}$5.0*10^{6}$}}%
      \put(976,3036){\makebox(0,0)[r]{\strut{}$1.0*10^{7}$}}%
      \put(976,3218){\makebox(0,0)[r]{\strut{}$1.5*10^{7}$}}%
      \put(976,3400){\makebox(0,0)[r]{\strut{}$2.0*10^{7}$}}%
      \put(976,3581){\makebox(0,0)[r]{\strut{}$2.5*10^{7}$}}%
      \put(976,3763){\makebox(0,0)[r]{\strut{}$3.0*10^{7}$}}%
      \put(976,3945){\makebox(0,0)[r]{\strut{}$3.5*10^{7}$}}%
      \put(976,4127){\makebox(0,0)[r]{\strut{}$4.0*10^{7}$}}%
      \put(1221,2512){\makebox(0,0){\strut{} 2}}%
      \put(1520,2512){\makebox(0,0){\strut{} 4}}%
      \put(1818,2512){\makebox(0,0){\strut{} 6}}%
      \put(2117,2512){\makebox(0,0){\strut{} 8}}%
      \put(2415,2512){\makebox(0,0){\strut{} 10}}%
      \put(2714,2512){\makebox(0,0){\strut{} 12}}%
      \put(3012,2512){\makebox(0,0){\strut{} 14}}%
      \put(3311,2512){\makebox(0,0){\strut{} 16}}%
      \put(128,3399){\rotatebox{-270}{\makebox(0,0){\strut{}operations/second}}}%
      \put(2191,2272){\makebox(0,0){\strut{}nr. of threads}}%
      \put(1184,3909){\makebox(0,0)[l]{\strut{}100\% Search}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(4576,2672){\makebox(0,0)[r]{\strut{}$0.0*10^{0}$}}%
      \put(4576,2963){\makebox(0,0)[r]{\strut{}$5.0*10^{6}$}}%
      \put(4576,3254){\makebox(0,0)[r]{\strut{}$1.0*10^{7}$}}%
      \put(4576,3545){\makebox(0,0)[r]{\strut{}$1.5*10^{7}$}}%
      \put(4576,3836){\makebox(0,0)[r]{\strut{}$2.0*10^{7}$}}%
      \put(4576,4127){\makebox(0,0)[r]{\strut{}$2.5*10^{7}$}}%
      \put(4821,2512){\makebox(0,0){\strut{} 2}}%
      \put(5120,2512){\makebox(0,0){\strut{} 4}}%
      \put(5418,2512){\makebox(0,0){\strut{} 6}}%
      \put(5717,2512){\makebox(0,0){\strut{} 8}}%
      \put(6015,2512){\makebox(0,0){\strut{} 10}}%
      \put(6314,2512){\makebox(0,0){\strut{} 12}}%
      \put(6612,2512){\makebox(0,0){\strut{} 14}}%
      \put(6911,2512){\makebox(0,0){\strut{} 16}}%
      \put(3728,3399){\rotatebox{-270}{\makebox(0,0){\strut{}operations/second}}}%
      \put(5791,2272){\makebox(0,0){\strut{}nr. of threads}}%
      \put(4784,3909){\makebox(0,0)[l]{\strut{}20\% Update}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(976,512){\makebox(0,0)[r]{\strut{}$0.0*10^{0}$}}%
      \put(976,694){\makebox(0,0)[r]{\strut{}$2.0*10^{6}$}}%
      \put(976,876){\makebox(0,0)[r]{\strut{}$4.0*10^{6}$}}%
      \put(976,1058){\makebox(0,0)[r]{\strut{}$6.0*10^{6}$}}%
      \put(976,1240){\makebox(0,0)[r]{\strut{}$8.0*10^{6}$}}%
      \put(976,1422){\makebox(0,0)[r]{\strut{}$1.0*10^{7}$}}%
      \put(976,1604){\makebox(0,0)[r]{\strut{}$1.2*10^{7}$}}%
      \put(976,1786){\makebox(0,0)[r]{\strut{}$1.4*10^{7}$}}%
      \put(976,1968){\makebox(0,0)[r]{\strut{}$1.6*10^{7}$}}%
      \put(1221,352){\makebox(0,0){\strut{} 2}}%
      \put(1520,352){\makebox(0,0){\strut{} 4}}%
      \put(1818,352){\makebox(0,0){\strut{} 6}}%
      \put(2117,352){\makebox(0,0){\strut{} 8}}%
      \put(2415,352){\makebox(0,0){\strut{} 10}}%
      \put(2714,352){\makebox(0,0){\strut{} 12}}%
      \put(3012,352){\makebox(0,0){\strut{} 14}}%
      \put(3311,352){\makebox(0,0){\strut{} 16}}%
      \put(128,1240){\rotatebox{-270}{\makebox(0,0){\strut{}operations/second}}}%
      \put(2191,112){\makebox(0,0){\strut{}nr. of threads}}%
      \put(1184,1750){\makebox(0,0)[l]{\strut{}50\% Update}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(6195,1745){\makebox(0,0)[r]{\strut{}$\Delta$Tree}}%
      \csname LTb\endcsname%
      \put(6195,1585){\makebox(0,0)[r]{\strut{}CBTree}}%
      \csname LTb\endcsname%
      \put(6195,1425){\makebox(0,0)[r]{\strut{}b$\Delta$Tree}}%
      \csname LTb\endcsname%
      \put(6195,1265){\makebox(0,0)[r]{\strut{}h$\Delta$Tree}}%
      \csname LTb\endcsname%
      \put(6195,1105){\makebox(0,0)[r]{\strut{}rbtree}}%
      \csname LTb\endcsname%
      \put(6195,945){\makebox(0,0)[r]{\strut{}avltree}}%
      \csname LTb\endcsname%
      \put(6195,785){\makebox(0,0)[r]{\strut{}sftree}}%
      \csname LTb\endcsname%
      \put(6195,625){\makebox(0,0)[r]{\strut{}NBBST}}%
      \csname LTb\endcsname%
      \put(6195,465){\makebox(0,0)[r]{\strut{}VTMTree}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./perf-4194303-eps-converted-to.pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> microbenchmarks.tex <==

\subsection{Microbenchmarks for Movidius Myriad1}
Regarding the assembly files used in the test execution process, a fix number of instructions in the loop was established for all the tests, meaning that each assembly file contains 5 instructions in the loop that is infinitely repeated. This convention was made in order to keep a continuity and a consistency of tests, by giving an insight in measuring the consumption on different SHAVE units, enabling to make comparisons between SHAVE units.
 
The assembly files used in the testing process, contain code that test the instruction power decode, instruction fetch. Majority of tests use pseudo-realistic data, by pseudo-realistic data we understand having as many non-zero values as possible and avoiding data value repetition at different offsets. 

Below are the used test cases as microbenchmark for Movidius platform.


\begin{itemize}

\item{SauMul, SauXor}:
 SAU operations - with instruction fetch and different data values (XOR-MUL)

\item{IauMul, IauXor}:
 IAU operations - with instruction fetch and different data values (XOR-MUL)

\item{VauMul, VauXor}:
 VAU operations - with instruction fetch and different data values (XOR-MUL)

\item{CmuCpss, CmuCpivr}:
 CMU operations --- with instruction fetch and different data values (CPSS - CPIVR)

\item{SauXorCmuCpss}:
 SAU \& CMU --- with instruction fetch and different data values (SAU.XOR $\|$ CMU.CPSS)

\item{SauXorCmuCpivr}:
 SAU \& CMU --- with instruction fetch and different data values (SAU.XOR $\|$ CMU.CPIVR)

\item{SauXorIauXor, IauXorCmuCpss}:
 SAU \& IAU --- with instruction fetch and different data values (SAU.XOR $\|$ IAU.XOR \& IAU.XOR $\|$ CMU.CPSS)

\item{SauXorVauXor, SauXorVauMul}:
 SAU \& VAU --- with instruction fetch and different data values (SAU.XOR $\|$ VAU.XOR \& SAU.XOR $\|$ VAU.MUL)

\item{SauXorCmuIauXor}:
 SAU \& IAU \& CMU --- with instruction fetch and different data values 
 (SAU.XOR $\|$ CMU.CPIS $\|$ IAU.XOR)
 
\end{itemize}

